Kleister: Key Information Extraction Datasets Involving Long Documents with Complex Layouts

The relevance of the Key Information Extraction (KIE) task is increasingly important in natural language processing problems. But there are still only a few well-defined problems that serve as benchmarks for solutions in this area. To bridge this gap, we introduce two new datasets (Kleister NDA and Kleister Charity). They involve a mix of scanned and born-digital long formal English-language documents. In these datasets, an NLP system is expected to find or infer various types of entities by employing both textual and structural layout features. The Kleister Charity dataset consists of 2,788 annual financial reports of charity organizations, with 61,643 unique pages and 21,612 entities to extract. The Kleister NDA dataset has 540 Non-disclosure Agreements, with 3,229 unique pages and 2,160 entities to extract. We provide several state-of-the-art baseline systems from the KIE domain (Flair, BERT, RoBERTa, LayoutLM, LAMBERT), which show that our datasets pose a strong challenge to existing models. The best model achieved an 81.77% and an 83.57% F1-score on respectively the Kleister NDA and the Kleister Charity datasets. We share the datasets to encourage progress on more in-depth and complex information extraction tasks.

==> results-data.tex <==
\toprule
\multicolumn{8}{c}{\emph{Kleister-NDA} dataset (pdf2djvu)} \\
\midrule
Entity name & \multicolumn{1}{l}{\textbf{Flair}} & \multicolumn{1}{l}{\textbf{BERT}} & \multicolumn{1}{l}{\textbf{RoBERTa}}&
\multicolumn{1}{l}{\textbf{LayoutLM}}&
\multicolumn{1}{l}{\textbf{LAMBERT}}&
\multicolumn{1}{l}{Autotagger}&
\multicolumn{1}{l}{Human}\\
\midrule
effective\_date & 79.37 & 80.20 & 81.50 & 82.08 & \textbf{85.27} & 79.00 & 100 \% \\
party & 70.13 & 71.60 & \textbf{80.83} & 75.28 & 78.70 & 33.15 & 98 \% \\
jurisdiction & 93.87 & 95.00 & 92.87 & 94.40 & \textbf{96.50} & 54.10 & 100 \% \\
term & \textbf{60.33} & 45.73 & 52.27 & 48.34 & 55.03 & 74.10 & 95 \% \\
\midrule
ALL & 77.83 & 78.20 & 81.00 & 78.68 & \textbf{81.77} & 60.09 & 97.86 \% \\
\toprule
\multicolumn{8}{c}{\emph{Kleister-Charity} dataset (Azure CV)} \\
\midrule
post\_town & \textbf{83.30} & 77.03 & 77.70 & 79.97 & 81.03 & 66.04 & 98 \% \\
postcode & 82.63 & 87.10 & \textbf{88.40} & 81.06 & 82.97 & 87.60 & 100 \% \\
street\_line & 68.17 & 62.23 & 72.03 & 70.92 & \textbf{75.33} & 75.02 & 96 \% \\
charity\_name  & 72.40 & 75.93 & 78.03 & 78.82 & \textbf{79.10} & 67.00 & 99 \% \\
charity\_number & \textbf{96.73} & 96.67 & 95.37 & 95.76 & 96.57 & 98.60 & 98 \% \\
income & 70.93 & 64.43 & 69.73 & 72.86 & \textbf{76.90} & 69.00 & 97 \% \\
report\_date & 95.67 & 96.60 & 96.77 & 95.42 & \textbf{95.80} & 89.00 & 100 \% \\
spending & 61.67 & 67.30 & 68.60 & 71.20 & \textbf{74.33} & 73.00 & 92 \% \\
\midrule
ALL & 80.10 & 78.33 & 81.50 & 80.74 & \textbf{82.97} & 78.16 & 97.45 \% \\
\bottomrule


\toprule
\multicolumn{8}{c}{\emph{Kleister-NDA} dataset (pdf2djvu)} \\
\midrule
Entity name & \multicolumn{1}{l}{\textbf{Flair}} & \multicolumn{1}{l}{\textbf{BERT}} & \multicolumn{1}{l}{\textbf{RoBERTa}}&
\multicolumn{1}{l}{\textbf{LayoutLM}}&
\multicolumn{1}{l}{\textbf{LAMBERT}}&
\multicolumn{1}{l}{Autotagger}&
\multicolumn{1}{l}{Human}\\
\midrule
effective\_date & 79.37 & 80.20 & 81.50 & 82.08 & \textbf{85.27} & 79.00 & 100 \% \\
party & 70.13 & 71.60 & \textbf{80.83} & 75.28 & 78.70 & 33.15 & 98 \% \\
jurisdiction & 93.87 & 95.00 & 92.87 & 94.40 & \textbf{96.50} & 54.10 & 100 \% \\
term & \textbf{60.33} & 45.73 & 52.27 & 48.34 & 55.03 & 74.10 & 95 \% \\
\midrule
ALL & 77.83 & 78.20 & 81.00 & 78.68 & \textbf{81.77} & 60.09 & 97.86 \% \\
\toprule
\multicolumn{8}{c}{\emph{Kleister-Charity} dataset (Azure CV)} \\
\midrule
post\_town & \textbf{83.30} & 77.03 & 77.70 & 79.97 & 81.03 & 66.04 & 98 \% \\
postcode & 82.63 & 87.10 & \textbf{88.40} & 81.06 & 82.97 & 87.60 & 100 \% \\
street\_line & 68.17 & 62.23 & 72.03 & 70.92 & \textbf{75.33} & 75.02 & 96 \% \\
charity\_name  & 72.40 & 75.93 & 78.03 & 78.82 & \textbf{79.10} & 67.00 & 99 \% \\
charity\_number & \textbf{96.73} & 96.67 & 95.37 & 95.76 & 96.57 & 98.60 & 98 \% \\
income & 70.93 & 64.43 & 69.73 & 72.86 & \textbf{76.90} & 69.00 & 97 \% \\
report\_date & 95.67 & 96.60 & 96.77 & 95.42 & \textbf{95.80} & 89.00 & 100 \% \\
spending & 61.67 & 67.30 & 68.60 & 71.20 & \textbf{74.33} & 73.00 & 92 \% \\
\midrule
ALL & 80.10 & 78.33 & 81.50 & 80.74 & \textbf{82.97} & 78.16 & 97.45 \% \\
\bottomrule

